DSText V2: A Comprehensive Video Text Spotting Dataset for Dense and Small Text

Recently, video text detection, tracking, and recognition in natural scenes are becoming very popular in the computer vision community. However, most existing algorithms and benchmarks focus on common text cases (e.g., normal size, density) and single scenario, while ignoring extreme video text challenges, i.e., dense and small text in various scenarios. In this paper, we establish a video text reading benchmark, named DSText V2, which focuses on Dense and Small text reading challenges in the video with various scenarios. Compared with the previous datasets, the proposed dataset mainly include three new challenges: 1) Dense video texts, a new challenge for video text spotters to track and read. 2) High-proportioned small texts, coupled with the blurriness and distortion in the video, will bring further challenges. 3) Various new scenarios, e.g., Game, Sports, etc. The proposed DSText V2 includes 140 video clips from 7 open scenarios, supporting three tasks, i.e., video text detection (Task 1), video text tracking (Task 2), and end-to-end video text spotting (Task 3). In this article, we describe detailed statistical information of the dataset, tasks, evaluation protocols, and the results summaries. Most importantly, a thorough investigation and analysis targeting three unique challenges derived from our dataset are provided, aiming to provide new insights. Moreover, we hope the benchmark will promise video text research in the community. DSText v2 is built upon DSText v1, which was previously introduced to organize the ICDAR 2023 competition for dense and small video text.

==> table/ablation_cross.tex <==
\def\x{{$\footnotesize \times$}}
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c|ccc}
    \whline
	\multirow{2}{*}{Train Set}   & 
	\multicolumn{3}{c}{Video Text Tracking/\%} 
	
    \cr\cline{2-4}  
    &  ${\rm ID_{F1}}$ & $\rm MOTA$& $\rm MOTP$ 
    \cr\shline \hline
	\hline
	
    
   ICDAR2015 (video)~\cite{karatzas2015icdar}
      & 49.9 & 32.3 & 72.2\\

   BOVText~\cite{wu2021bilingual}
      & 29.6 & 10.9& 74.5 \\

   COCOText~\cite{veit2016coco}
      & 43.4 & 27.9 & 79.0 \\

    DSText V2
   & 55.2 & 39.3 & 77.4 \\
     


     \whline
\end{tabular}


==> table/task1.tex <==
\def\x{{$\footnotesize \times$}}
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c|c|ccc|ccc|p{0.32\columnwidth}}
    \whline
	User ID  & Rank &  $\rm MOTA$& $\rm MOTP$ & ${\rm ID_{F1}}$/\% & 	M-M &  P-M & 	M-L &Affiliations \cr\shline \hline
	\hline
	TencentOCR
     & 1 & 	62.56\% & 79.88\% & 75.87\% & 8114	& 1800&	2663&	 Tencent. \\
     DA
     & 2 & 	50.52\% & 78.33\% & 	70.99\% & 7121	& 2405 &	3051&	 Guangzhou Shiyuan Electronic Technology Company Limited \\
     Tianyu Zhang
     & 3 & 		43.52\% & 78.15\% & 	62.27\% & 4980	& 2264 &	5333&	 AI Lab, Du Xiaoman Financial \\
     Liu Hongen
     & 4 & 		36.87\% & 79.24\% & 	48.99\% & 2123	& 3625 &	6829 &	 Tianjin Univeristy \\
     Yu Hao
     & 5 & 		31.01\% & 78.00\% & 		50.39\% & 2361	& 1767 &	8449 &	 - \\
     Hu Jijin
     & 6 & 		28.92\% & 78.46\% & 		43.96\% & 1385	& 1186 &	10006 &	 Beijing University of Posts \& Telecommunications \\
     	CccJ
     & 7 & 		27.55\% & 78.40\% & 		44.28\% & 1583	& 1103 &	9891 &	 CQUT \\
     MiniDragon
     & 8 & 		25.75\% & 	74.03\% & 		50.22\% & 3302	& 2806 &	6469 &	 - \\
     FanZhengDuo
     & 9 & 		23.41\% & 	75.54\% & 			49.66\% & 5216	& 3578 &	3783 &	 - \\
     zjb
     &10 & 		19.85\% & 		71.98\% & 			39.87\% & 2815	& 3354 &	6408 &	 - \\
     dunaichao
     &11 & 		19.84\% & 		73.82\% & 			31.18\% & 924	& 1765 &	9888 &	 China Mobile Communications Research Institute \\
     JiangQing
     &12 & 		13.83\% & 		75.75\% & 			58.41\% & 6924	& 2622 &	3031 &	 South China University of Technology; Shanghai AI Laboratory; KingSoft Office CV\&D Department \\
     Kebin Liu
     &13 & 			7.49\% & 		75.62\% & 		45.68\% & 5403		& 3835 &	3339 &	 Beijing University of Posts and Telecommunications \\
     TungLX &14 & 			0\% & 		0\% & 		0\% & 0		& 0 &	0 &	 - \\
     \whline
\end{tabular}


==> table/task2.tex <==
\def\x{{$\footnotesize \times$}}
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c|c|ccc|ccc|p{0.3\columnwidth}}
    \whline
	User ID  & Rank &  $\rm MOTA$& $\rm MOTP$ & ${\rm ID_{F1}}$/\% & 	M-M &  P-M & 	M-L &Affiliations \cr\shline \hline
	\hline
	TencentOCR
     & 1 & 	22.44\% & 80.82\% & 56.45\% & 5062	& 1075&	6440&	 Tencent. \\
     DA
     & 2 & 		10.51\% & 78.97\% & 	53.45\% & 4629	& 1392 &	6556&	 Guangzhou Shiyuan Electronic Technology Company Limited \\
     dunaichao
     &3 & 		5.54\% & 		74.61\% & 			24.25\% & 528	& 946 &	11103 &	 China Mobile Communications Research Institute \\
 	cnn\_lin &4 & 		0\% & 		0\% & 			0\% & 0	& 0 &	0 &	 South China Agricultural University \\
 	Hu Jijin &5 & 		0\% & 		0\% & 			0\% & 0	& 0 &	0 &	 Beijing University of Posts and Telecommunications \\
 	XUE CHUHUI &6 & 		0\% & 		0\% & 			0\% & 0	& 0 &	0 &	 - \\
 	MiniDragon &7 & 		-25.09\% & 		74.95\% & 			26.38\% & 1388	& 1127 &	10062 &	 - \\
 	JiangQing
     &8 & 		-27.47\% & 		76.59\% & 			43.61\% & 4090	& 1471 &	7016 &	 South China University of Technology; Shanghai AI Laboratory; KingSoft Office CV\&D Department \\
     Tianyu Zhang
     & 9 & 		-28.58\% & 80.36\% & 		26.20\% & 1556	& 543 &	10478&	 AI Lab, Du Xiaoman Financial \\
     \whline
\end{tabular}

